Physics-guided Learning-based Adaptive Control on the SE(3) Manifold

In real-world robotics applications, accurate models of robot dynamics are critical for safe and stable control in rapidly changing operational conditions. This motivates the use of machine learning techniques to approximate robot dynamics and their disturbances over a training set of state-control trajectories. This paper demonstrates that inductive biases arising from physics laws can be used to improve the data efficiency and accuracy of the approximated dynamics model. For example, the dynamics of many robots, including ground, aerial, and underwater vehicles, are described using their $SE(3)$ pose and satisfy conservation of energy principles. We design a physically plausible model of the robot dynamics by imposing the structure of Hamilton's equations of motion in the design of a neural ordinary differential equation (ODE) network. The Hamiltonian structure guarantees satisfaction of $SE(3)$ kinematic constraints and energy conservation by construction. It also allows us to derive an energy-based adaptive controller that achieves trajectory tracking while compensating for disturbances. Our learning-based adaptive controller is verified on an under-actuated quadrotor robot.

==> tex/AdaptiveControl.tex <==
\section{Adaptive Control}
\label{sec:adaptive_control}
\begin{itemize}
\item Using meta learning seems interesting and related \cite{richards21adaptive}: \url{http://www.roboticsproceedings.org/rss17/p056.pdf}. They only consider external forces as unknown variables. We can have changing mass, inertia, and external forces like winds?
\item Their problem formulation is summarized below ( Eq. (11) in their paper \cite{richards21adaptive}).
\begin{equation}
\begin{aligned}
&\min_{\theta} \frac{1}{NMT} \left( \sum_{i = 1}^N \sum_{j=1}^M \int_0^T c_{ij}(t)dt + \mu_{meta} \Vert \theta \Vert^2_2 \right)\\
s.t. \quad & c_{ij} = \Vert x_{ij} - r_i \Vert ^2_2 + \alpha \Vert u_ij\Vert^2_2 \\
& \dot{x}_{ij} = \hat{f}_j(x_{ij}, u_{ij}; \psi_j), x_{ij}(0) = r_i(0), \\
& u_{ij} = \pi(x_{ij}, r_i, a_{ij}; \theta_\pi),\\
& \dot{a} = \rho(x_{ij}, r_i, a_{ij}, \theta_\rho), a_{ij}(0) = 0.
\end{aligned}
\end{equation}
\item We already have the controller $\pi$. \TODO{We need to learn a adaptation rule $\rho$ for the unknown mass, inertia and/or external force in Hamiltonian formulation.} They use a neural network as the function $\rho$ and try to update its parameters $\theta_\rho$ using meta learning framework.
\item Our framework can learn the approximated dynamics function $\hat{f}_j$ for each $j$th sample of the disturbances (mass, inertia or external forces).
\item They only used one step approximation instead of using ODE solver. We can use the ODE solver here.
\item They cited this paper \cite{slotine1987adaptive} for tracking convergence. Does it still hold for our case? They only considered a fully actuated system while ours is under-actuated.
\end{itemize}

==> tex/Preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelim}
%\subsection{Learning Hamiltonian dynamics on the SE(3) manifold}
%\begin{itemize}
%	\item Let $\mathbf\frakq = [\bfp^\top \quad \bfr_1^\top \quad \bfr_2^\top \quad \bfr_3^\top]^\top \in \mathbb{R}^{12}$ be the generalized coordinates, and $\bfzeta = [\bfv^\top\!\quad \bfomega^\top]^\top \in \mathbb{R}^6$ be the generalized velocity. Note that $\mathbf\frakq$ and $\bfzeta$ have different dimensions and satisfy the $SE(3)$ kinematics constraints, re-expressed in vectorized form as:
%	%
%	\begin{equation}
%	\label{eq:pose_kinematics_rewritten}
%	\dot{\mathbf\frakq} = \mathbf\frakq^{\times}\mathbf\bfzeta, \qquad \mathbf\frakq^{\times} = \begin{bmatrix}
%	\bfR^\top\!\!\!\! & \bf0 & \bf0 & \bf0 \\
%	\bf0 & \hat{\bfr}_1^\top & \hat{\bfr}_2^\top & \hat{\bfr}_3^\top
%	\end{bmatrix}^\top.
%	\end{equation}
%	\item Given a dataset $\calD$ with no disturbances, we learn the Hamiltonian dynamics of the robot on the SE(3) manifold, i.e. we learn the mass $\bfM^{-1}_\phi$, the potential energy $V_\phi$ and the input matrix $\bfg_\phi$. The dynamics $\bff_\phi$ of the state $\bfx$ is governed by the Hamilton's equations:
%	\begin{equation}
%	\label{eq:port_Hal_dyn}
%	\begin{bmatrix}
%	\dot{\mathbf\frakq} \\
%	\dot{\mathbf\frakp} \\
%	\end{bmatrix}
%	= (\mathbf\calJ(\mathbf\frakq, \mathbf\frakp) - \mathbf\calR(\mathbf\frakq, \mathbf\frakp))
%	\begin{bmatrix}
%	\frac{\partial \mathcal{H}}{\mathbf\frakq} \\
%	\frac{\partial \mathcal{H}}{\mathbf\frakp} 
%	\end{bmatrix} + \mathbf\calG(\mathbf\frakq, \mathbf\frakp)\bfu,
%	\end{equation}
%	where
%	\begin{equation}
%	\label{eq:SE3_PH_J}
%	\bf\mathcal{J}(\mathbf\frakq, \mathbf\frakp) = \begin{bmatrix}
%	\bf0 & \mathbf\frakq^{\times} \\
%	-\mathbf\frakq^{\times\top} & \mathbf\frakp^{\times} 
%	\end{bmatrix}, \qquad \mathbf\frakp^{\times} = \begin{bmatrix}
%	\bf0 & \hat{\mathbf\frakp}_{\bfv}\\
%	\hat{\mathbf\frakp}_{\bfv} & \hat{\mathbf\frakp}_{\bfomega}
%	\end{bmatrix},
%	\end{equation}
%	\item To collect the dataset $\calD$, we can use a PID controller like in our RSS paper.
%	\item Given this dynamics, we already derived a trajectory tracking controller $\bfu = \bfmu_{IDA-PBC} (\bfx, \bfr; \phi)$ in our RSS paper.
%	\item \TODO{Comments: The learned Hamiltonian dynamics does not account for the disturbances, i.e. $\hat{\bff}(\bfx, \bfu, \bf0;\bfphi)$ only.}
%	\item With the disturbance modeled in Eq. \eqref{eq:f_external}, the Hamiltonian dynamics becomes:
%		\begin{equation}
%	\label{eq:port_Hal_dyn_disturbance}
%	\begin{bmatrix}
%	\dot{\mathbf\frakq} \\
%	\dot{\mathbf\frakp} \\
%	\end{bmatrix}
%	= (\mathbf\calJ(\mathbf\frakq, \mathbf\frakp) - \mathbf\calR(\mathbf\frakq, \mathbf\frakp))
%	\begin{bmatrix}
%	\frac{\partial \mathcal{H}}{\mathbf\frakq} \\
%	\frac{\partial \mathcal{H}}{\mathbf\frakp} 
%	\end{bmatrix} + \mathbf\calG(\mathbf\frakq, \mathbf\frakp)\bfu + \bff_e,
%	\end{equation}
%\end{itemize}

%
%\subsection{Hamiltonian formulation for robot dynamics on the SE(3) manifold}
%\label{subsec:ham_dyn}
% 
%where \begin{equation}
%\label{eq:approx_tracking_cost}
%\hat{\calC} = \frac{1}{NMT} \left( \sum_{i = 1}^N \sum_{j=1}^M \int_0^T c(\bfx_{ij}(t), \bfr_j(t), \bfu_{ij}(t)) \right).
%\end{equation}
%
%\begin{itemize}
%	\item Given $N$ desired trajectories $\{\bfx^*_i(t)\}^N_{i=1}$ and $M$ samples of the disturbances $\{\bfw_j\}_{j=1}^N$.
%	\item The parameter $\bftheta$ in the adaptive controller (Eq. \eqref{eq:adaptive_controller}) is optimized via meta-learning:
%	\begin{equation}
%	\label{eq:ac_ml_truedyns}
%	\begin{aligned}
%	&\min_{\bftheta} \frac{1}{NMT} \left( \sum_{i = 1}^N \sum_{j=1}^M \int_0^T c_{ij}(t)dt + \mu_{meta} \Vert \bftheta \Vert^2_2 \right)\\
%	s.t. \quad & c_{ij} = \Vert \bfx_{ij} - \bfx^*_i \Vert ^2_2 + \bfalpha \Vert \bfu_{ij}\Vert^2_2 \\
%	& \dot{\bfx}_{ij} = {\bff}(\bfx_{ij}, \bfu_{ij}, \bfw_j), \bfx_{ij}(0) = \bfx^*_i(0), \\
%	& \bfu_{ij} = \bfpi(\bfx_{ij}, \bfx^*_i, \bfa_{ij}; \bftheta_\pi),\\
%	& \dot{\bfa} = \bfrho(\bfx_{ij}, \bfx^*_i, \bfa_{ij}, \bftheta_\rho), \bfa_{ij}(0) = \bf0.
%	\end{aligned}
%	\end{equation}
%	\item However, the true dynamics  ${\bff}(\bfx_{ij}, \bfu_{ij}, \bfw_j)$ cannot be simulated online because of the unknown disturbance $\bfw_j$ and its effect on the dynamics.
%	\item The initial controller in Eq. \eqref{eq:init_controller} is used to collect state-control dataset $\calD_j$. Then, the true dynamics  ${\bff}(\bfx_{ij}, \bfu_{ij}, \bfw_j)$ is approximated by $\hat{\bff}(\bfx_{ij}, \bfu_{ij}; \bfxi_j)$ with parameter $\bfxi_j$ for each $\bfw_j$.
%	\item The meta-learning problem becomes:
%		\begin{equation}
%	\label{eq:ac_ml_approxdyns}
%	\begin{aligned}
%	&\min_{\bftheta} \frac{1}{NMT} \left( \sum_{i = 1}^N \sum_{j=1}^M \int_0^T c_{ij}(t)dt + \mu_{meta} \Vert \bftheta \Vert^2_2 \right)\\
%	s.t. \quad & c_{ij} = \Vert \bfx_{ij} - \bfx^*_i \Vert ^2_2 + \bfalpha \Vert \bfu_{ij}\Vert^2_2 \\
%	& \dot{\bfx}_{ij} = \hat{\bff}(\bfx_{ij}, \bfu_{ij}; \bfxi_j), \bfx_{ij}(0) = \bfx^*_i(0), \\
%	& \bfu_{ij} = \bfpi(\bfx_{ij}, \bfx^*_i, \bfa_{ij}; \bftheta_\pi),\\
%	& \dot{\bfa} = \bfrho(\bfx_{ij}, \bfx^*_i, \bfa_{ij}, \bftheta_\rho), \bfa_{ij}(0) = \bf0.
%	\end{aligned}
%	\end{equation}
%	\item The ensemble $\{\hat{\bff}(\bfx_{ij}, \bfu_{ij}; \bfxi_j)\}_{j=1}^M$ represents the distribution of ${\bff}(\bfx_{ij}, \bfu_{ij}, \bfw_j)$ over the disturbance $\bfw$.
%	\item \TODO{Comments: The adaptive control framework via meta learning in \cite{richards21adaptive} is general. Then, the authors apply the framework on  fully-actuated Lagrangian systems as the form of the adaptive law $\bfrho$ in Eq. \eqref{eq:adaptive_controller} for this kind of system is derived by Slotine and Li \cite{slotine1987adaptive}. We can try their form of the function $\bfrho$ as well but we don't have proof that the same adaptive law will converge to the right value of the unknown $\bfa$ as our states lie on the SE(3) manifold. Also, the quadrotor in our paper is an under-actuated system. The next section will describe a geometric adaptive law for states on SE(3) manifold.}
%\end{itemize}

%\begin{itemize}
%	\item Goodarzi et al. \cite{goodarzi2015geometric} propose a geometric adaptive controller for trajectory tracking on the SE(3) manifold.
%	\item The disturbance $\bff_e$ in Eq. \eqref{eq:f_external} is split into external force and torque:
%		\begin{equation}
%	\label{eq:f_tau_external}
%	\begin{aligned}
%	\bff_{e} &= \bfW_\bfp(\bfx)\bfa_\bfp,\\
%	\bftau_{e} &= \bfW_\bfR(\bfx)\bfa_\bfR,\\
%	\end{aligned}
%	\end{equation}
%	\item The adaptive law for attitude tracking:
%	\begin{equation}
%	\label{eq:adaptive_law_attitude}
%	\dot{\bfa}_{\bfR} = \gamma_{\bfR} \bfW_{\bfR}^\top (e_{\bfomega} + c_{\bfR} e_{\bfR})
%	\end{equation}
%	where $e_\bfR = \frac{1}{2}(\bfR^{*\top} \bfR - \bfR^\top \bfR^*)^\vee$ and $e_{\bfomega} = \bfomega - \bfR^T \bfR^* \bfomega^*$.
%	\item The adaptive law for position tracking:
%	\begin{equation}
%	\label{eq:adaptive_law_position}
%	\dot{\bfa}_{\bfp} = \gamma_{\bfp} \bfW_{\bfp}^\top (e_{\bfv} + c_{\bfp} e_{\bfp})
%	\end{equation}
%	where $e_\bfp = \bfp - \bfp^*$ and $e_\bfv = \bfv - \bfv^*$. 
%	\item \TODO{Comments: The adaptive laws are actually very similar to the law used in \cite{richards21adaptive}. The difference is that the errors are defined	 on the SE(3) manifold. Plus, Goodarzi et al. \cite{goodarzi2015geometric} proved the stability of the adaptive controller with the Lee's controller \cite{lee2010geometric}. As our IDA-PBC controller is connected with the Lee's controller, should we aim to prove stability with our IDA-PBC controller as well? Or just using the above adaptive laws in the meta-learning framework (Eq. \eqref{eq:ac_ml_approxdyns}) is good enough?}
%
%\end{itemize}

==> tex/RelatedWork.tex <==
\section{Related Work}
\label{sec:related_work}
%\begin{enumerate}
%	\item \textbf{Adaptive Control.}
%		\begin{itemize}
%			\item General adaptive control: adaptive law: \cite{narendra2012stable, ioannou2012robust}
%			\item Linearly parameterizable dynamics, i.e. the external force can be express in linear form of a feature matrix. \cite{slotine1987adaptive, slotine1989composite, slotine1991applied}
%			\item Adaptive control for Hamiltonian dynamics: \cite{nageshrao2015port, dirksz2012structure, slotine1990hamiltonian, dirksz2010adaptive}
%			\item Adaptive control for SE(3) manifold: \cite{goodarzi2015geometric, dydek2012adaptive, selfridge2014multivariable, antonelli2017adaptive, zhen2013adaptive, cabecinhas2014nonlinear, lee2009feedback, bialy2013lyapunov}, Check reference from lee's paper.
%		\end{itemize}
%	\item \textbf{Meta Learning}
%		\begin{itemize}
%			\item General meta learning: cite Chelsea Finn's papers \cite{finn2017model} + survey \cite{hospedales2020meta}.
%		\end{itemize}
%	\item \textbf{Learning A Controller}
%		\begin{itemize}
%			\item General dynamics and/or control learning: learn dynamics first and then control, or learn control directly.
%			\item 
%			\item learning control for port-hamiltonian system: \cite{nageshrao2015port}
%			\item Adaptive control via meta learning: learn control + adaptively update some internal disturbance state online \cite{o2021meta, shi2021meta, harrison2018control, harrison2018meta, rajeswaran2016epopt, belkhale2021model, lee2019meta}. Learn the feature matrix using neural nets \cite{joshi2019deep,joshi2020asynchronous}, GP \cite{sanner1991gaussian, gahlawat20al1adaptive, grande2013nonparametric}
%		\end{itemize}
%\end{enumerate}



Adaptive control designs aim to tolerate parametric, structural, or disturbance uncertainties while achieving system stability and asymptotic tracking. A recent comprehensive survey is presented in \cite{tao2014adaptive}. Commonly, an adaptation law is an augmentation of an existing nominal controller that adjusts the controller parameters based on performance errors. Self-tuning control (STC) and model reference adaptive control (MRAC) are the two most popular adaptive control methods for linear systems. A key technical issue in nonlinear adaptive control is the parameterization of the system uncertainties \cite{krstic1995nonlinear}. For linearly parameterized systems, disturbances are modeled as linear combinations of known nonlinear features and updated by an adaptation law based on the state errors with stability obtained by, e.g., sliding-mode theory \cite{slotine1987adaptive, slotine1989composite, slotine1990hamiltonian, slotine1991applied, dirksz2012structure, dirksz2010adaptive}, assuming zero-state detectability \cite{sastry1989adaptive, dirksz2012structure, dirksz2010adaptive} or $\calL1-$adaptation \cite{hovakimyan2010L1, gahlawat20al1adaptive,hanover2021performance}. For mechanical systems, such adaptation laws are paired with a nominal controller, derived using Lagrangian dynamics with feedback linearization \cite{slotine1987adaptive, slotine1989composite, slotine1990hamiltonian, slotine1991applied, dirksz2012structure, dirksz2010adaptive}, Hamiltonian dynamics with energy shaping \cite{nageshrao2015port, dirksz2012structure, dirksz2010adaptive}, or model predictive control \cite{adetola2009adaptive,heirung2017dual, lorenzen2017adaptive,pereida2018adaptive,hanover2021performance}. Meanwhile, if the systems evolve on a manifold, e.g., $SE(3)$, an adaptition law is designed based on geometric errors, derived from the manifold constraints \cite{fernando2011robust,lee2012robust, goodarzi2015geometric,bisheban2018geometric, bisheban2020geometric}.


%
%\TODO{\NA{re-write this second part of the sentence}resulting in adaptive laws often derived by sliding mode theory \cite{slotine1987adaptive, slotine1989composite, slotine1990hamiltonian, slotine1991applied}. \NA{This transition from linearly parameterized systems to port-Hamiltonian systems is too abrupt}For (port-)Hamiltonian dynamical systems \cite{van2014port}, Dirksz and Scherpen \cite{nageshrao2015port, dirksz2012structure, dirksz2010adaptive} proposed an adaptive controller based on the output of the system, assuming zero-state detectability of the system. \NA{There does not seem to be much structure to this paragraph. The sentences are too disconnected.}For systems on the $SE(3)$ manifold such as quadrotors, several adaptive controllers have been proposed for known robot dynamics based on linearization \cite{slotine1990hamiltonian, dydek2012adaptive, selfridge2014multivariable, bialy2013lyapunov}, simplified models \cite{antonelli2017adaptive, zhen2013adaptive}, and sliding mode \cite{lee2009feedback}. Also, Bisheban and Lee \cite{bisheban2020geometric} used a three-layer neural network to model the disturbance but derive adaptive law for the network's parameters instead of learning from data.}\NA{This part needs to be improved.}




%Adaptive control \cite{krstic1995nonlinear, narendra1989stable, ioannou1996robust} has been widely used to design regulation and tracking controllers that adapt to disturbances and parameter uncertainties. The trajectory tracking controller is often developed based on a nominal dynamics, e.g. via Lagrangian dynamics with feedback linearization, and compensates for the disturbances, estimated online by an adaptive control law. 



%Recently, there has been a growing interest in learning a controller from data. An indirect approach is to learn the robot dynamics from data while imposing certain prior knowledge on the structure of the model, e.g. neural networks \cite{lutter2019deeplagrangian, zhong2020symplectic, duong21hamiltonian}. The model structure is then used to derive a closed-loop controller for trajectory tracking. On the other hand, a controller can also be learned directly from data and guarantee system stability \cite{sun2020learning, chang2020neural, Dai21Lyapunov, khansari2011learning} \TD{Relevant but not very related to adaptive control. Remove this?}. 

Recently, there has been growing interest in applying machine learning techniques to design adaptive controllers. Since the nonlinear disturbance features are actually unknown in practice, they can be estimated using Gaussian processes \cite{sanner1991gaussian, gahlawat20al1adaptive, grande2013nonparametric} or neural networks \cite{joshi2019deep,joshi2020asynchronous, harrison2018control, o2021meta, richards21adaptive}. The features can be learned from data online in the control loop \cite{gahlawat20al1adaptive, joshi2019deep,joshi2020asynchronous}, which is potentially too slow for real-time operation, or offline via meta-learning from past state-control trajectories \cite{o2021meta, harrison2018control, harrison2018meta} or simulation of the system dynamics \cite{richards21adaptive}. Given the learned disturbance features, an adaptation law is designed to estimate the disturbances online, e.g. using $\calL_1$ adaptation \cite{gahlawat20al1adaptive} or by updating the last layer of the feature neural networks \cite{joshi2019deep,joshi2020asynchronous, o2021meta, harrison2018control, richards21adaptive, shi2021meta}. Besides the disturbance features, the parameters of the adaptive controllers can be learned as well using meta-learning \cite{richards21adaptive}. 

%  based on sliding mode theory \cite{utkin2013sliding}

%Recently, there has been a growing interest in learning an adaptive controller from data, which focuses on deriving a trajectory tracking controller and learning the nonlinear features characterizing the external force.  To learn this adaptive law, the nonlinear features are learned online in the control loop \cite{gahlawat20al1adaptive, joshi2019deep,joshi2020asynchronous}, which potentially suffers from slow feature update/training, or offline  via meta-learning from pre-collected data \cite{o2021meta, harrison2018control, harrison2018meta} and from offline simulation of an approximated dynamics learned from pre-collected trajectories \cite{richards21adaptive}. 

%Meta-learning \cite{finn2017model, hospedales2020meta} is originally proposed for learning control policies that work for different tasks in model-based reinforcement learning setting \cite{rajeswaran2016epopt, clavera2018model, belkhale2021model} and for nonlinear systems \cite{harrison2018meta, o2021meta, shi2021meta, richards21adaptive}. In this framework, there are base-learners, one for solving each task, and a meta-learner that optimizes meta-parameters, i.e. shared among the base-learners, by back-propagating the gradient of a meta-objective function. Several recent works have been re-framing adaptive control problem as a meta-learning problem and solve for the optimal parameters. Specifically, 
%Harrison et. al \cite{harrison2018meta, harrison2018control} model the robot dynamics by a neural network with the last layer acting as weights in a Bayesian framework. The network's parameters and the prior distribution over the last layer's weights are updated using meta-learning with offline pre-collected data. Online control adaptation is then achieved via Bayesian linear regression and an iLQR controller. Both O'Connell et. al. \cite{o2021meta} and Richards et. al \cite{richards21adaptive}, instead, assume a known nominal Lagrangian dynamics with unknown an external force approximated by a neural network. However, while the former work learns the external force via meta-learning with pre-collected trajectories, the latter does that by simulating trajectories from an approximated dynamics function learned beforehand from data. Then, an adaptive controller is derived based on the approximated external forces via feedback linearization. Meanwhile, Shi et. al \cite{shi2021meta} also propose an online meta-adaptive control framework that learns a shared representation of the unknown dynamics caused by disturbances and provides convergence guarantees for both meta-learning and adaptive control provided that the loss function is convex. 

While prior learning-based adaptive control techniques \cite{joshi2019deep,joshi2020asynchronous, o2021meta, harrison2018control, richards21adaptive, shi2021meta} rely on Lagrangian dynamics and feedback linearization to design the adaptive trajectory tracking controller, we approach the control design  from an energy perspective using Hamiltonian dynamics on the $SE(3)$ manifold. Compared to adaptive controllers for quadrotors with known $SE(3)$ dynamics \cite{fernando2011robust,lee2012robust, goodarzi2015geometric,bisheban2018geometric, bisheban2020geometric}, we develop a general adaptation law based on geometric tracking errors with a disturbance model learned from trajectory data that can be used for any rigid-body robot, such as a UGV, UAV, or UUV.
% and UUV, via Hamiltonian formulation.

%an adaptive law based on geometric tracking errors,  inspired by \cite{goodarzi2015geometric}, and disturbance model learned from past state-control trajectories that can be used for any single-body robots, such as UGV, UAV and UUV, via Hamiltonian formulation.


%Inspired by \cite{richards21adaptive}, we propose to learn an adaptive controller via meta-learning for Hamiltonian dynamics on the SE(3) manifold. Instead of using a nominal model, we learn a Hamiltonian dynamics, which accounts for the external force and respects the SE(3) constraints, completely from data. Given the Hamiltonian formulation, we derive an adaptive controller using energy-based approach with an adaptive law for SE(3) manifold inspired by \cite{goodarzi2015geometric}. Similar to \cite{richards21adaptive}, we also simulate the dynamics offline and use meta-learning framework to optimize the controller's parameters which can be used for under-actuated systems on the SE(3) manifold like quadrotor.
%The gradient is back-propagated through ridge regression \cite{lee2019meta,harrison2018meta}
%
%\subsection{Adaptive Control via Meta Learning}
%Richards et. al \cite{richards21adaptive} solve Problem \ref{prob:control_learning} for vector-valued state $\bfx \in \bbR^n$ via the meta-learning framework described in Sec. \ref{subsec:meta_learning}. Specifically, given $N$ reference trajectories $\{\bfr_i(t)\}_{i=1}^N$ with $M$ samples of the disturbance $\{\bfw_j\}_{j=1}^M$, the tracking cost $\calC$ is approximated by 
%\begin{equation}
%\hat{\calC} = \frac{1}{NMT} \left( \sum_{i = 1}^N \sum_{j=1}^M \int_0^T c(\bfx_{ij}(t), \bfr_j(t), \bfu_{ij}(t))dt \right),
%\end{equation}
%where $c(\bfx_{ij}, \bfr_j, \bfu_{ij}) = \Vert \bfx_{ij} - \bfr_j\Vert^2_2 + \alpha \Vert \bfu_{ij} \Vert_2^2$ and $\alpha$ is some coefficient. The Problem \ref{prob:control_learning} is reformulated as a meta-learning problem as follows.
%\begin{problem}
%	\label{prob:control_metalearning}
%	Find an adaptive controller of the form $(\bfpi, \bfrho)$ that minimizes the approximated tracking cost $\hat{\calC}$ over the parameter $\bftheta = \{\bftheta_\bfpi, \bftheta_\bfrho\}$:
%	\begin{equation}
%	\label{eq:approx_cost_problem}
%	\begin{aligned}
%	&\bftheta^* = {\arg\min}_\bftheta \hat{\calC} \\
%	s.t. \quad & \dot{\bfx}_{ij} = {\bff}(\bfx_{ij}, \bfu_{ij}, \bfw_j), \bfx_{ij}(0) = \bfx^*_i(0), \\
%	& \bfu_{ij} = \bfpi(\bfx_{ij}, \bfx^*_i, \bfa_{ij}; \bftheta_\pi),\\
%	& \dot{\bfa}_{ij} = \bfrho(\bfx_{ij}, \bfx^*_i, \bfa_{ij}, \bftheta_\rho), \bfa_{ij}(0) = \bf0, \\
%	& i = 1, \ldots, N, j = 1, \ldots, M,
%	\end{aligned}
%	\end{equation}
%	where each pair $k=(i,j)$ of the reference trajectory $\bfr_i(t)$ and the disturbance $\bfw_j$ is considered a task $k$, the meta-learner's parameter and loss function $\calL^m$ are $\bftheta$ and $\hat{\calC}$, respectively, and the base learner's parameter for the task $(i,j)$ is $\bfpsi_{ij} = \{\bfx_{ij}, \bfu_{ij}, \bfa_{ij}\}$. 
%\end{problem}
%
%Since the effect of the disturbance $\bfw$, i.e. $\bff_\bfw$ on the robot dynamics is unknown, true dynamics  ${\bff}(\bfx, \bfu, \bfw_j)$ is approximated by $\hat{\bff}(\bfx, \bfu; \bfxi_j)$ with parameter $\bfxi_j$ for each $\bfw_j$. Under the disturbance $\bfw_j$, a dataset $\calD_j = \{t^{(d)}_{0:1}, \bfx^{(d)}_{0:1}, \bfu^{(d)}\}_{d = 0}^{D_j-1}$ is collected and used to train the model $\hat{\bff}(\bfx, \bfu; \bfxi_j)$  by minimizing the loss function:
%\begin{equation}
%\label{eq:disturbance_dyn_learning}
%\begin{aligned}
%&\min_{\bfzeta_j} \sum_{k = 1}^{D_j} \ell(\bar{\bfx}(t^{(d)}_1), \bfx^{(d)}_{1})   \\
%s.t. \quad & \dot{\bar{\bfx}} = \hat{\bff}(\bar{\bfx}, \bfu^{(d)}, \bfxi_j), \bar{\bfx}(0) = \bfx^{(d)}_0,
%\end{aligned}
%\end{equation} 
%where the loss $\ell(\bar{\bfx}(t^{(d)}_1), \bfx^{(d)}_{0})$ represents the discrepancy between the data point $\bfx^{(d)}_{1}$ and its approximation $\bar{\bfx}(t^{(d)}_1)$.
%
%The Problem \ref{prob:control_metalearning} is then solved for a fully actuated Lagrangian dynamical systems, i.e. $\bff$ function, with state $\bfx = [\frakq, \dot{\frakq}]$ where $\frakq \in \bbR^n$ and $\dot{\frakq} \in \bbR^n$ are the generalized coordinate and its velocity, respectively. The controller $\bfpi$ is derived using feedback linearization and the adaptive law $\bfrho$ is inspired from Slotine and Li's adaptive controller  \cite{slotine1987adaptive} for fully actuated systems. However, the generalized coordinate $\frakq$ is a real vector in $\bbR^n$. In our setting, the coordinate $\frakq$ lies on the SE(3) manifold and the dynamical system $\bff$ described in Hamiltonian formulation is possibly under-actuated, e.g. quadrotor, and learned completely from data.


